TweetEval: Unified Benchmark and Comparative Evaluation for Tweet Classification

The experimental landscape in natural language processing for social media is too fragmented. Each year, new shared tasks and datasets are proposed, ranging from classics like sentiment analysis to irony detection or emoji prediction. Therefore, it is unclear what the current state of the art is, as there is no standardized evaluation protocol, neither a strong set of baselines trained on such domain-specific data. In this paper, we propose a new evaluation framework (TweetEval) consisting of seven heterogeneous Twitter-specific classification tasks. We also provide a strong set of baselines as starting point, and compare different language modeling pre-training strategies. Our initial experiments show the effectiveness of starting off with existing pre-trained generic language models, and continue training them on Twitter corpora.

==> oldtables.tex <==
\section{Number of tokens per datasets}

Table \ref{table-tokenizer} includes number of chars per tweet for each of the tasks and the difference between word pieces of the pre-trained RoBERTa-base and RoBERTa trained from scratch, which apply the Byte-Pair Encoding (BPE) tokenizer \cite{sennrich2015neural}.
This is useful to understand if a model recognizes more or less tokens: if the number is high, it means that the model had to split more times a word.

\begin{table}[h]
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{3.0pt}
\scalebox{0.85}{ 
\begin{tabular}{lcccc}
\toprule
\textbf{Task} & \textbf{Chars} & \textbf{RoB-RT} & \textbf{RoB-Tw} & \textbf{\% Diff} \\ \midrule
Emoji &  71.3 {\small $\pm$21} & 22.4 {\small $\pm$7.4} & 21.6 {\small $\pm$6.9} & 2.9 {\small $\pm$6.9}  \\
Emotion &  90.9 {\small $\pm$36.8} & 27.2 {\small $\pm$10.2} & 25.8 {\small $\pm$9.7} & 5.2 {\small $\pm$8.1}  \\
Hate &  132.6 {\small $\pm$72.5} & 38.7 {\small $\pm$19.8} & 36.1 {\small $\pm$18.9} & 6.9 {\small $\pm$8.2}  \\
Irony &  85.2 {\small $\pm$31.7} & 26.1 {\small $\pm$9.3} & 25.1 {\small $\pm$9} & 3.8 {\small $\pm$7.2}  \\
Sentiment &  95.7 {\small $\pm$127.8} & 26.7 {\small $\pm$9.2} & 26.3 {\small $\pm$9.1} & 1.4 {\small $\pm$8.5}  \\
Offensive &  144.8 {\small $\pm$78} & 42 {\small $\pm$21} & 39.5 {\small $\pm$19.7} & 5.7 {\small $\pm$8.6}  \\
S/Abortion  &  107.5 {\small $\pm$25.5} & 31.2 {\small $\pm$7.7} & 31 {\small $\pm$7.4} & 0.4 {\small $\pm$5.3}  \\
S/Atheism &  105.9 {\small $\pm$26.4} & 31.3 {\small $\pm$7.9} & 31.1 {\small $\pm$7.7} & 0.5 {\small $\pm$4.4}  \\
S/Climate &  106.9 {\small $\pm$23.7} & 30.1 {\small $\pm$6.3} & 30.6 {\small $\pm$6.6} & -1.6 {\small $\pm$5.1}  \\
S/Feminist &  105.9 {\small $\pm$25.2} & 30.5 {\small $\pm$7.3} & 29.9 {\small $\pm$7} & 1.7 {\small $\pm$5}  \\
S/Hilary &  106 {\small $\pm$21.8} & 30.9 {\small $\pm$6.5} & 30.4 {\small $\pm$6.2} & 1.5 {\small $\pm$4.6}  \\
\bottomrule
\end{tabular}
}
\caption{\label{table-tokenizer} Statistics from each task of \textsc{TweetEval}.
``Chars'' is the average number of characters in each tweet, RoB-RT and Rob-Tw are the average number of word pieces after tokenization with the original Roberta-base tokenizer and with the trained from scratch tokenizer. ``Diff'' is the the percentile difference of tokens in each tweet between these two tokenizers (if the difference is positive, the original RoBERTa includes more tokens.) }

\end{table}
